Kino-PAX: Highly Parallel Kinodynamic Sampling-based Planner

Sampling-based motion planners (SBMPs) are effective for planning with complex kinodynamic constraints in high-dimensional spaces, but they still struggle to achieve real-time performance, which is mainly due to their serial computation design. We present Kinodynamic Parallel Accelerated eXpansion (Kino-PAX), a novel highly parallel kinodynamic SBMP designed for parallel devices such as GPUs. Kino-PAX grows a tree of trajectory segments directly in parallel. Our key insight is how to decompose the iterative tree growth process into three massively parallel subroutines. Kino-PAX is designed to align with the parallel device execution hierarchies, through ensuring that threads are largely independent, share equal workloads, and take advantage of low-latency resources while minimizing high-latency data transfers and process synchronization. This design results in a very efficient GPU implementation. We prove that Kino-PAX is probabilistically complete and analyze its scalability with compute hardware improvements. Empirical evaluations demonstrate solutions in the order of 10 ms on a desktop GPU and in the order of 100 ms on an embedded GPU, representing up to 1000 times improvement compared to coarse-grained CPU parallelization of state-of-the-art sequential algorithms over a range of complex environments and systems.

==> sections_final/CUDA_computing.tex <==
% \qh{For my reference, can you write in bullet points what are the main considerations for motion planning with CUDA GPU and how \alg is optimized for that?}

% \np{
% \begin{itemize}
%    \item Balance workloads across threads; i.e., avoid conditional statements that lead to expensive subroutines. In \alg, each subroutine ensures that every thread follows nearly the same execution path. Functions like \texttt{PropagateFrontier}, \texttt{UpdateEstimates}, and \texttt{UpdateTreeSearch} exhibit minimal thread divergence. Although \texttt{PropagateFrontier} has some divergence for collision checking, this is necessary to efficiently collect data, and outside of this, each thread performs nearly identical calculations. An example of poor workload balance would be to continuously propagate samples until all have hit a collision. This approach causes some threads to propagate for a very long time, resulting in idle threads and bottlenecking the GPU workload.
%     \item Avoid sequential algorithms that require multiple GPU calls, as each call requires synchronization, which can be costly. Examples of such algorithms include sorting, finding the shortest path, or managing a min-heap (managing samples organized by their region in $\mathcal{R}$).
%     \item Design GPU functions (kernels) to allow threads to operate independently as much as possible. For example, in \alg, during sample propagation, the acceptance of a sample is independent of the samples made by other threads. A poor design choice would be to select the best \textit{n} samples, which requires costly comparisons across threads.
%     \item Optimize the memory layout on the GPU to minimize footprint and ensure efficient access patterns. For instance, \alg uses a 1D array for $\mathcal{T}$ to manage memory efficiently and reduce overhead during memory reads and writes. A poor memory layout example would be organizing samples based on their region, which would require a very large sparse array. Such an array would be expensive to access due to scattered memory access patterns, leading to inefficient use of memory bandwidth and increased latency during propagation.
%     \item Minimize data transfers between the device (GPU) and the CPU to reduce latency and improve performance. \alg manages all large data structures entirely on the device, only sending minimal information, such as a \texttt{solution found flag} and \texttt{frontier size}, to the CPU. By limiting these data transfers, \alg reduces latency between GPU kernel calls and avoids bottlenecks caused by the PCIe bus bandwidth limitations (bandwidth between GPU and CPU).
% \end{itemize}
% }

% We now present a brief overview of CPU and GPU architecture, providing insight into the motivation for redesigning and moving Kinodynamic SBMPs to GPU devices. 

\ml{Not sure if this section is necessary.  All of it can be summarized into one paragraph, which can become the first paragraph of the algorithm section.  We can keep this section for the extended version of the paper.}

This work focuses on designing a highly parallel kinodynamic sampling-based algorithm, with particular focus on development for the many thousand core architectures of GPUs. Thus, a general understanding of the execution hierarchies of such devices in contrast to traditional CPUs is essential, as it influences core components of the algorithm design. 

The design approach of traditional multicore CPU devices is commonly referred to as a \emph{latency-oriented design} \cite{kirk2016programming}, meaning it is optimized for executing sequential code with minimal delay between each operation. However, parallelism is possible and prevalent on modern CPU devices, but due to the design emphasis on higher-clock speeds, the amount of concurrency is limited. On the other hand, the design of many-thread GPUs take an alternative approach, with the goal of maximizing the amount of chip area dedicated for floating-point calculations and memory access throughput. GPUs optimize for parallelism of a massive number of threads, rather than reducing the latency of individual threads. These design choices are well-suited for the problem discussed in section \ref{sec:problem}, as subroutines such as trajectory segment propagation or validity checking can be executed as a highly concurrent process.

To better understand the design of a successful parallel algorithm, we briefly discuss the structure of GPU execution. GPUs operate using a three-level hierarchy. At the lowest level are \emph{warps}, which consist of groups of 32 threads that execute the same instruction simultaneously on different data. If threads within a warp follow divergent execution paths, such as those caused by conditional statements, some threads become idle, reducing efficiency.  Therefore, it is essential that our parallel algorithm minimizes uneven workloads across the device to maintain high occupancy and better performance.

The next level of the GPU hierarchy consists of \emph{blocks}, which are groups of threads that can share data through a small amount of on-chip memory. This memory enables fast communication and synchronization among threads within the same block. However, threads from different blocks cannot share memory directly. Therefore, it is crucial to maximize block independence to minimize the need for device-wide synchronization. Additionally, we must optimize the use of shared memory within blocks to take advantage of the low-latency resources available.

Finally, at the highest level, blocks are organized into grids, which are dispatched to the device for execution. In summary, an algorithm well-suited for parallelization should have the following qualities: \emph{independence between threads}, \emph{even workloads across threads}, and \emph{effective utilization of available low-latency memory} \cite{guide2020cuda}. 
 
% In this work, we focus on designing a highly parallel kinodynamic sampling-based algorithm, with particular focus on development for the many thousand core architecture of GPUs. To achieve efficient performance on these high-throughput devices, it is crucial that our algorithm complements the GPU execution hierarchy to optimize resource utilization and ease of implementation. For the development of this algorithm, we follow the guidance of \cite{kirk2016programming} and \cite{guide2020cuda} and consider the following principles:

% \begin{itemize} 
%     \item \emph{Thread independence} — The ability for each thread in a program to execute without being dependent on the state or result of other threads.
%     \item \emph{Even workloads across threads} — Each thread is assigned an equal or nearly equal number of operations throughout its execution.
%     \item \emph{Utilization of low-latency memory} —  Groups of threads utilize low-latency memory to share information and reduce the number of higher-latency global memory accesses.
% \end{itemize}

% With these principles in mind, we propose \alg, ...

% \qh{Discuss the parts of the parallel architecture that warrants requiring: every thread follows the same execution path: balance workload across threads}

% A highly parallel algorithm comes another consideration: sparsity. \qh{if tree size is too large, will slow down: sparsitiy}

% \qh{Finally, stress that these points are general for highly parallel algorithm...}


% \qh{We may want to summarize some of this in bullet points or bold?}


% Thus, before committing to parallelizing an algorithm, the original problem must be decomposed into its independent sections to be determined if it is worth the added overhead.

% We now present a brief overview of CPU and GPU architecture, providing insight into the motivation for redesigning and moving Kinodynamic SBMPs to GPU devices. Additionally, we cover the functional hierarchy of NVIDIA-specific CUDA-enabled GPUs which \alg exploits and much of its design is based upon. A more detailed description of all topics discussed in this section can be found in \cite{kirk2016programming}.

% \subsection{Multicore CPUs and Many-thread GPUs}

% The design approach of traditional multicore CPU devices is commonly referred to as a \textit{latency-oriented design}, meaning it is optimized for executing sequential code with minimal delay between each operation. To achieve this, CPUs provide large on-chip memory caches and apply internal algorithms to minimize idle resources. While these strategies effectively reduce the time required for individual operations, they also increase the chip's area and power consumption.

% In contrast, the design of many-thread GPUs take an alternative approach, with the goal of maximizing the amount of chip area dedicated for floating-point calculations and memory access throughput. GPUs optimize for parallelism of a massive number of threads, rather than reducing the latency of individual threads. The result is a processor that is easily amenable to scale-out techniques, steadily improving in throughput performance as CPU clock speed optimizations have become relatively stagnant.

% For the problem considered in \ref{sec:problem}, which generally deals with high-dimensional state spaces and lacks steering functions, the number of required trajectory segments to find a solution grows exponentially with dimensionality. Consequently, the amount of floating-point operations also increases exponentially, making GPUs a particularly enticing candidate for handling such problems. This necessitates the design of kinodynamic SBMP algorithms specifically optimized to exploit the capabilities of GPU technology.

% \np{possibly move this content to the introduction? I would like to give an intuition of why it is worth the headache of decomposing existing serial algorithms and translating them for GPUs. Also, this lends well to high dimensional state space problems where we require many samples (i.e many floating point ops) to find a solution. }

% \subsection{CUDA Enabled GPUs}

% To design an efficient algorithm for GPU devices, a general understanding of the device specific execution hierarchy is essential, as it influences core components of the algorithm design. Specifically, this work focuses on CUDA-enabled GPUs. These GPUs operate using a three-level execution hierarchy. At the lowest level are \emph{warps}, which consist of groups of 32 threads that execute the same instruction simultaneously on different data. If threads within a warp follow divergent execution paths, such as those caused by conditional statements, some threads become idle, reducing efficiency. The next level of the CUDA hierarchy consists of blocks, which are groups of threads that can share data through a small amount of on-chip shared memory. This memory enables fast communication and synchronization among threads within the same block. However, threads from different blocks cannot share memory directly. Finally, at the highest level, blocks are organized into grids, where they are dispatched to the device for execution.

% While CUDA-enabled GPUs offer significant throughput compared to CPU devices, they also come with limitations. As noted by \cite{thomason2024motions}, utilizing GPUs incurs memory transfer overhead between the device and the host machine. Additionally, certain algorithms, such as sorting, are not easily parallelizable, which can result in multiple GPU calls to obtain the final solution. Thus, before committing to parallelizing an algorithm, the original problem must be decomposed into its independent sections to be determined if it is worth the added overhead.

% Parallelizing SBMPs has been long studied with success of traditional roadmap based algorithms such as PRM being demonstrated to be ``embarrassingly" parallel \cite{amato1999probabilistic}, i.e approximately 100\% of the algorithm can be parallelized. On the other hand, tree based planners such as RRT have proven less trivial for paralleization implementations as the nearest neighbor checking and extension method are inherently sequential thus many parallel calls. 

% When designing algorithms for CUDA-enabled devices, it is crucial to carefully consider the inherent limitations of GPUs. Additionally, the problem must be decomposed into independent pieces . Additionally, certain types of algorithms are inherently sequential, making them poorly suited for GPU execution \qh{can we say that RRT, EST, and all the other sampling-based algorithms are inherently sequential?}. 

% \np{PRM style planners are not inherently sequential. In RRT the nearest neighbor subroutine is, also tree expansion is sequential and not easily parallelizable. EST propagation is also sequential and maintaining probability of expansion for each node is non trivial.}

% To mitigate these challenges, it is essential to minimize both the amount and frequency of data transferred between the CPU and GPU, ensuring that only necessary data is communicated. Furthermore, achieving independence between threads and balancing computational loads across them is vital for maximizing GPU efficiency. By doing so, the overhead of data communication can be justified by the significant gains in throughput.

% The fundamental architectural differences between GPU and CPU computing.

% \alg is designed with these limitations in mind, to leverage the strength of massive parallelism of the GPU architecture. \alg minimizes thread divergence through careful construction of subroutines, limits the amount and frequency of data transferred between the CPU and GPU, and avoids inherently hard-to-parallelize functions commonly found in SBMP algorithms.

==> sections_final/KGMT.tex <==

% The efficiency of the search in KGMT depends on the tree's ability to rapidly expand in all space dimensions. To achieve this, KGMT employs a high-level discrete representation of the tree’s exploration progress in each region, effectively guiding its expansion in all directions. When the low-level motion planner has accurate data on search progress, the many-core architecture of the GPU can be better leveraged to outwardly expand the tree as a massively parallel process. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/G-EST.pdf}
    \caption{Caption for the image}
    \label{fig:G-EST}
\end{figure}

% \qh{Need to say that these promising regions are used to add the frontier in parallel and not selected. This current writing sounds like a normal motion planning alg, not a GPU one}


% \np{
% \begin{itemize}
%    \item Balance workloads across threads; i.e., avoid conditional statements that lead to expensive subroutines. In \alg, each subroutine ensures that every thread follows nearly the same execution path. Functions like \texttt{PropagateFrontier}, \texttt{UpdateEstimates}, and \texttt{UpdateTreeSearch} exhibit minimal thread divergence. Although \texttt{PropagateFrontier} has some divergence for collision checking, this is necessary to efficiently collect data, and outside of this, each thread performs nearly identical calculations. An example of poor workload balance would be to continuously propagate samples until all have hit a collision. This approach causes some threads to propagate for a very long time, resulting in idle threads and bottlenecking the GPU workload.
%     \item Avoid sequential algorithms that require multiple GPU calls, as each call requires synchronization, which can be costly. Examples of such algorithms include sorting, finding the shortest path, or managing a min-heap (managing samples organized by their region in $\mathcal{R}$).
%     \item Design GPU functions (kernels) to allow threads to operate independently as much as possible. For example, in \alg, during sample propagation, the acceptance of a sample is independent of the samples made by other threads. A poor design choice would be to select the best \textit{n} samples, which requires costly comparisons across threads.
%     \item Optimize the memory layout on the GPU to minimize footprint and ensure efficient access patterns. For instance, \alg uses a 1D array for $\mathcal{T}$ to manage memory efficiently and reduce overhead during memory reads and writes. A poor memory layout example would be organizing samples based on their region, which would require a very large sparse array. Such an array would be expensive to access due to scattered memory access patterns, leading to inefficient use of memory bandwidth and increased latency during propagation.
%     \item Minimize data transfers between the device (GPU) and the CPU to reduce latency and improve performance. \alg manages all large data structures entirely on the device, only sending minimal information, such as a \texttt{solution found flag} and \texttt{frontier size}, to the CPU. By limiting these data transfers, \alg reduces latency between GPU kernel calls and avoids bottlenecks caused by the PCIe bus bandwidth limitations (bandwidth between GPU and CPU).
% \end{itemize}
% }

% \qh{every thread follows the same execution path: balance workload across threads}

% \qh{avoid sequential steps}

% \qh{allow threads to operate independently as much as possible: acceptance of sample}

% \qh{optimize memory layout}

% \qh{minimize data transfers}

% \qh{if tree size is too large, will slow down}

% \qh{sparsitiy of tree}


We propose \alg, a kinodynamic sampling-based motion planning algorithm designed to take advantage of the capabilities of CUDA-enabled devices. \alg grows a tree of trajectory segments directly on the GPU. Our key insight is that each iteration of the tree growth process (i.e., selection of nodes, extension, validity checking, and adding new nodes to the tree) can be made independent, enabling efficient parallelization. Additionally, \alg minimizes communication between the CPU and GPU, ensures balanced workloads across threads, and avoids inherently sequential subroutines.

At each iteration of \alg, a set of nodes in the tree are expanded in parallel. Each sample is extended multiple times through random sampling of controls, also in parallel. We dynamically adjust the number of extensions in each iteration to maintain an effective tree growth rate, ensuring efficient usage of the GPU device's throughput. After extension, a new set of nodes are selected as samples independently.

To guide the search process, \alg employs a high-level space decomposition approach that is well suited for parallel computation. The decomposition estimates the exploration progress made in each region, and identifies promising regions to select nodes for extension and adding new nodes to the tree. \qh{Need to add a sentence to give a hint on why the approach is suited for GPUs} As more trajectory segment data becomes available, the decomposition is refined \qh{what do you mean by the decomposition being refined?}, allowing \alg to focus on propagating a large number of promising samples into unexplored areas of the space.

% By directing which tree samples to propagate from in future parallel expansions, the algorithm effectively manages the growth of the tree.

% In early iterations, when the tree is relatively small, each sample undergoes numerous extensions to rapidly expand the search space and jumpstart the tree growth process. As the size of the tree increases, \alg reduces the number of extensions per sample to prevent the serialization of operations due to device throughput limitations. 

% To guide this process, a high-level space decomposition is used to estimate the exploration progress within each discrete region of the space. This decomposition identifies promising regions for new sample acceptance and directing future node expansions. As the tree iteratively grows in a massively parallel process, new information on valid and invalid trajectories guides \alg in determining where to focus the next parallel expansion.

% The design of \alg considers the key points discussed in Section \ref{sec:CUDA_computing} to develop a novel kinodynamic motion planning algorithm that efficiently utilizes GPU resources. 

% \alg operates by generating trajectory segments in parallel, using a set of samples known as the frontier. Each sample is extended a number of  times to better utilize the device's throughput. \alg operates by expanding multiple nodes in parallel, simultaneously branching the tree in all relevant directions within the search space.



% The resulting structure resembles a breadth-first search, with branches flooding outward in all directions of the state space simultaneously.

\subsection{Core Algorithm}

A pseudocode of \alg is shown in Alg.~\ref{algo: alg}, with subroutines Algs.~\ref{algo: PropagateFrontier}, \ref{algo:UpdateEstimates}, and \ref{algo:UpdateTreeSearch}. A visualization of a full planning iteration is shown in Fig.~\ref{fig:iteration_grid}.

In Alg.~\ref{algo: alg}, \texttt{\alg} takes as input the initial agent state $x_{init}$, a goal region $X_{goal}$, and a maximum execution time $t_{max}$. In lines 1-3, the sample set $V_F$ is initialized with the state $x_{init}$ and the sets $V_{unexplored}$ and $V_{open}$ are initialized as empty. Additionally, a tree $\mathcal{T}$ is initialized with $x_{init}$ at its root. The sets—$V_{unexplored}$, $V_{open}$, and $V_F$—partition the samples of $\mathcal{T}$ into three distinct sections, with each sample belonging to one of these sets. This partitioning facilitates efficient memory management where each set is represented by a boolean mask over $\mathcal{T}$.

The set $V_{unexplored}$ consists of newly generated samples that have not yet been added to the tree. The set $V_{open}$ includes samples that are not currently considered for expansion; intuitively, these samples are located in densely populated or frequently invalid regions of the state space. Finally, $V_F$ represents the current frontier of the tree, comprising samples that are set for parallel expansion.

Next, in lines 4-5 of Alg.~\ref{algo: alg}, the space decomposition \(\mathcal{R}\) and a fine overlaid decomposition \(\mathcal{R}_2\) are initialized. These decompositions can be defined in either the workspace \(\mathcal{W}\) or the state space \(X\). In the state space, the decomposition consists of non-overlapping regions, such that:

\[
X = \mathcal{R}_1 \cup \mathcal{R}_2 \cup \dots \cup \mathcal{R}_n \quad \text{and},
\]
\[
\quad \forall \mathcal{R}_i, \mathcal{R}_j \in X, \; \text{Interior}(\mathcal{R}_i) \cap \text{Interior}(\mathcal{R}_j) = \emptyset.
\]

Each state \(x \in X \) is uniquely associated with a region \(\mathcal{R}_i\) using the function \(\texttt{getRegion}(x)\), which maps \(x\) to \(\mathcal{R}_i\) if and only if \(x \in \mathcal{R}_i\). Decompositions can be constructed using various techniques, such as simple grids or triangulations. For simplicity, all experiments conducted in this paper use a grid-based decomposition.


For each region $\mathcal{R}_i \in \mathcal{R}$, several metrics are calculated to assess the exploration progress of the tree $\mathcal{T}$. These metrics, adapted from the work of \cite{plaku2010motion}, are designed to be effective in identifying promising regions for systems with complex dynamics and are well suited for GPU parallelism. Specifically, $\alg$ updates the following metrics for each region, $\mathcal{R}_i$, after each expansion iteration to continually guide the search process:

\begin{itemize} \item \textbf{$Cov(\mathcal{R}_i)$} — estimates the progress made by the sampling-based motion planner in covering $\mathcal{R}_i$; \item \textbf{$FreeVol(\mathcal{R}_i)$} — estimates the free volume of $\mathcal{R}_i$. \end{itemize}


Based on these metrics, a sample acceptance probability, denoted as $\mathbf{Accept}(\mathcal{R}_i)$, is calculated to determine the likelihood of adding a newly generated sample within region $\mathcal{R}_i$ to the tree $\mathcal{T}$. This probability also determines whether a sample located in the set $V_{open}$ will be moved to the set $V_F$ for propagation in the next iteration of the parallel tree expansion.

Once the space decomposition has been initialized, the main loop of the algorithm begins, covering lines 7-11. In line 7, the \texttt{PropagateFrontier} function is called to propagate the set $V_F$ in parallel. The subroutine for this process is detailed in \ref{algo: PropagateFrontier}, with the pseudocode being a serialized version of the GPU implementation.

In \texttt{PropagateFrontier}, each sample of $V_F$, denoted by $x_0$ on line 1, is expanded $\lambda$ times. The parameter $\lambda$, known as the branching factor, controls the amount of parallelism when expanding $V_F$. This parameter must be carefully managed to efficiently utilize the throughput offered by the GPU. A low $\lambda$ (e.g., $\lambda \rightarrow 1$) leads to faster propagation iterations and a sparser tree but underutilizes the GPU's throughput when $V_F$ is small. Conversely, a high $\lambda$ (e.g., $\lambda \rightarrow 32$) allows the tree to expand rapidly, making better use of the GPU. However, as $V_F$ grows, the propagation requirements may exceed the GPU’s capacity, causing operations to become serialized. To optimize $\lambda$ based on the specific device and problem dynamics, a tuning value $t_e$, referred to as the expected tree size, is introduced. This value adjusts $\lambda$ for each iteration of parallel expansion. In early iterations, when the tree size $t$ is much smaller than $t_e$, a larger $\lambda$ is used to maximize parallelism and speed up tree propagation. As the tree size $t$ approaches $t_e$ and $V_F$ is large, a smaller $\lambda$ is employed to prevent serialization of the propagation process. If the tree size exceeds $t_e$, $t_e$ is updated to accommodate the growing tree and maintain effective parallel expansion.

We now move to the logic for each thread and its corresponding sample $x_0$ in \texttt{PropagateFrontier}, covered in lines 3-10 of \ref{algo: PropagateFrontier}. Line 3 handles the propagation of the sample and generates a new state, $x_1$. Then in line 4, the corresponding regions of $x_1$, $\mathcal{R}_i$ and $\mathcal{R}2_j$ are calculated. In lines 5-8, the trajectory from $x_0$ to $x_1$ is checked for validity. If the trajectory is valid, the total number of valid samples located in region $\mathcal{R}_i$ is incremented. Additionally, if the sub-region $\mathcal{R}2_j$ is unvisited, or based on the probability determined by \textbf{$\text{Accept}(\mathcal{R}_i)$}, the sample is added to the set $V_{unexplored}$. Conversely, if the sample is found to be invalid, the count of invalid samples in region $\mathcal{R}_i$ is incremented, as shown in line 10.

After all frontier samples have been expanded, the values of \textbf{$Cov(\mathcal{R}_i)$}, \textbf{$FreeVol(\mathcal{R}_i)$}, and \textbf{$Accept(\mathcal{R}_i)$} are updated in parallel for each region in $\mathcal{R}$, in line 8 of \ref{algo: alg} and detailed in subroutine \ref{algo:UpdateEstimates}, \texttt{UpdateEstimates}. On line 2 of the subroutine, each thread independently updates its free volume using the following equation:

\begin{equation}
\label{eq:FreeVol}
\text{FreeVol}(\mathcal{R}_i) = \frac{\epsilon + n_{valid}(\mathcal{R}_i)}{\epsilon + n_{valid}(\mathcal{R}_i) + n_{invalid}(\mathcal{R}_i)} \times \text{vol}(\mathcal{R}_i)
\end{equation}

where $\epsilon > 0$ is a small user-defined constant, and $vol(\mathcal{R}_i)$ represents the workspace volume of region $\mathcal{R}_i$. Next, on line 3 of  \texttt{UpdateEstimates}, the coverage score of each region, \textbf{$Cov(\mathcal{R}_i)$}, is updated by counting the number of $\mathcal{R}2$ cells within $\mathcal{R}_i$ that contain samples from $\mathcal{T}$. Once these metrics have been updated for all regions in $\mathcal{R}$, the acceptance probability \textbf{$\text{Accept}(\mathcal{R}_i)$} is calculated in parallel using the following equations:

\begin{equation}
\label{eq:Accept}
\text{Accept}(\mathcal{R}_i) = \frac{\mathcal{R}_i.w}{\sum_{\mathcal{R}_j \in \mathcal{R}_{\text{avail}}} \mathcal{R}_j.w} + \epsilon
\end{equation}

\begin{equation}
\label{eq:R_iw}
\mathcal{R}_i.w = \frac{\text{FreeVol}^4(\mathcal{R}_i)}{(1 + \text{Cov}(\mathcal{R}_i))(1 + (n_{valid}(\mathcal{R}_i) + n_{invalid}(\mathcal{R}_i))^2)}
\end{equation}

Here, $\mathcal{R}_{\text{avail}}$ represents the set of regions $\mathcal{R}_{avail} \in \mathcal{R}$ that contain a sample in $\mathcal{T}$.

Once the \textbf{$\text{Accept}(\mathcal{R}_i)$} probabilities have been updated for all regions, the \texttt{UpdateTreeSearch} subroutine is called on line 9 of \ref{algo: alg}. In \texttt{UpdateTreeSearch} shown by algorithm \ref{algo:UpdateTreeSearch}, lines 1-4 remove samples from the frontier set $V_F$ with a probability corresponding to 1 - \textbf{$\text{Accept}(\mathcal{R}_i)$}, ensuring that promising samples remain in the frontier. Lines 5-8 move all samples from the unexplored set $V_{unexplored}$ to $V_F$ and check for goal criteria on line 7, returning the valid trajectory $\gamma$ if the goal is found. Finally, lines 9-12 move inactive samples in $V_{open}$ to the frontier if they are now deemed promising with the updated search information. Once all samples in $\mathcal{T}$ have been placed in the correct sample partition, the subroutine exits and \alg continues until a user-defined time limit $t_{max}$ is surpassed or when a trajectory $\gamma$ is returned by \texttt{UpdateTreeSearch}.






% \subsection{High-Level Discrete Model}

% The high-level discrete model provides a simplified representation of the progress made by the underlying motion planner within each region. This data can then be used by the motion planner to extend from promising nodes and accept new nodes in less explored regions. These regions can be defined in either the workspace represented by $\mathcal{W}$ or the state space denoted by $\mathcal{S}$. KGMT allows for use of either representation and the performance impact of these decomposition choices are studied in Section [BLANK].

% Throughout the paper the decomposition will be assumed to be made in the state-space $\mathcal{S}$ and is defined by the non-overlapping regions, i.e., $\mathcal{S} = \mathcal{R}_1 \cup \mathcal{R}2 \cup \dots \cup \mathcal{R}_n$, where a state $s \in \mathcal{S}$ can be mapped to a region $\mathcal{R}_i$ with $\forall s \in \mathcal{S} : \text{getRegion}(s) = \mathcal{R}_i \text{ iff } s \in \mathcal{R}_i$. Various methods can be employed for space decomposition, as it remains an active area of research.
% Techniques such as simple grids or triangulations are commonly used; however, for all the experiments conducted in this paper, a grid-based decomposition was chosen.

% To measure the exploration progress of the tree $\mathcal{T}$, two metrics are used from SyCLoP, each designed for efficient computation and are shown to be effective in estimating promising regions for systems with complex dynamics. Specifically, for each region $\mathcal{R}_i$ the following metrics are calculated:
% \begin{itemize}
%     \item \textbf{$Cov(\mathcal{R}_i)$} estimates the progress made by sampling-based motion planner in covering $\mathcal{R}_i$;
%      \item \textbf{$FreeVol(\mathcal{R}_i)$} estimates the free volume of $\mathcal{R}_i$;
% \end{itemize}

% The metric \textbf{$Cov(\mathcal{R}_i)$} estimates the coverage of a region $\mathcal{R}_i$ by the tree $\mathcal{T}$. To efficiently compute \textbf{$Cov(\mathcal{R}_i)$}, \textit{KGMT} overlays an implicit grid, denoted as $\mathcal{R}2$, onto the space. It then counts the number of $\mathcal{R}2$ cells within $\mathcal{R}_i$ that contain samples from $\mathcal{T}$. The grid $\mathcal{R}2$ is set to a fine resolution to allow for accurate coverage estimates. Throughout the experiments in this paper, the grid is set to be twice as fine as the higher-level grid $\mathcal{R}$. Calculations for the coverage of each region is performed after each iteration of parallel tree expansion.

% The free volume of a region, \textbf{$freeVol(\mathcal{R}_i)$}, provides \textit{KGMT} with an estimate of the difficulty in exploring that particular region. Regions with a higher free volume are generally easier to explore compared to those with a smaller free volume. The free volume for each region is updated after each iteration of parallel tree expansion by the following equation:

% \begin{equation*}
%     \text{FreeVol}(\mathcal{R}_i) = \frac{ \epsilon + n_{valid}(\mathcal{R}_i)}{\epsilon + n_{valid}(\mathcal{R}_i) + n_{invalid}(\mathcal{R}_i)} * vol(\mathcal{R}_i)
% \end{equation*}
% where $\epsilon > 0$ is a small user-defined constant and $vol(\mathcal{R}_i)$ is the workspace volume of $\mathcal{R}_i$.

% With these two metrics, a probability for each region, denoted by \textbf{$\text{Accept}(\mathcal{R}_i)$}, is calculated after each iteration of parallel tree expansion. This probability represents the likelihood that a tree sample within region \textbf{$\mathcal{R}_i$} will be selected for propagation in the next iteration of parallel expansion. Additionally, \textbf{$\text{Accept}(\mathcal{R}_i)$} determines the probability that newly generated samples are added to the tree \textbf{$\mathcal{T}$}. This probability is calculated by the following equation:

% \[
% \frac{\mathcal{R}_i.w}{\sum_{\mathcal{R}_j \in \mathcal{R}_{\text{avail}}} \mathcal{R}_j.w}
% \]

% \[
% \mathcal{R}_i.w = \frac{\text{FreeVol}^4(\mathcal{R}_i)}{(1 + \text{Cov}(\mathcal{R}_i))(1 + (n_{valid}(\mathcal{R}_i) + n_{invalid}(\mathcal{R}_i))^2)}
% \]
% where $\mathcal{R}_{\text{avail}}$ represents the set of regions $\mathcal{R}_{avail} \in \mathcal{R}$ that contain a sample in $\mathcal{T}$.

% KGMT's space decomposition is inspired by SyCLoP; however, KGMT modifies the discrete representation and tree expansion estimation to better leverage the parallelism offered by GPUs. Specifically, edges between regions are not considered and the Single-Source Shortest Path (SSSP) problem from $\mathcal{R}_{init}$ to  $\mathcal{R}_{goal}$ is not solved. The removal of these complexities is well-suited to GPU implementation, as tree samples within all available regions can be expanded in parallel, better utilizing the massive throughput of modern GPUs. Additionally, KGMT avoids the inherently sequential SSSP problem which becomes a bottleneck as the space decomposition becomes finer.

% Unlike SyCLoP, KGMT does not use a high-level plan, such as a sequence of connecting regions from $\mathcal{R}{\text{init}}$ to $\mathcal{R}{\text{goal}}$. In SyCLoP, this plan guides the tree search towards the goal, effectively creating a depth-first search. The rationale for KGMT's approach is rooted in the architecture of GPUs, which excels at massive parallelism in non-sequential operations. Restricting propagation to regions within a high-level plan would generally underutilize the throughput of modern GPUs. Additionally, a high-level plan is a depth-frist search which inheritently requires sequential propagations from regions $\mathcal{R}{\text{init}}$ to $\mathcal{R}{\text{goal}}$. Moreover, the SSSP problem that SyCLoP solves to determine the high-level plan is a sequential operation that does not benefit significantly from GPU acceleration unless the decomposition is extremely fine [SOURCE]. By removing this complexity, KGMT allows all tree samples to be considered for propagation, better utilizing GPU throughput and enabling finer decompositions that more effectively guides tree propagation.

% \subsection{Core Algorithm}

% We now detail the \textit{KGMT} algorithm which utilizes the high-level space decomposition. This algorithm iteratively attempts to expand all samples in $\mathcal{T}$, with the probability of expansion for each sample determined by the region to which it belongs. The core part of \textit{KGMT} proceeds by repeating the following steps until a solution is found:

% \begin{itemize}
%     \item Use the estimates of \textbf{$\text{FreeVol}(\mathcal{R}_i)$} and \textbf{$\text{Cov}(\mathcal{R}_i)$} to calculate \textbf{$\text{Accept}(\mathcal{R}_i)$} for each region in $\mathcal{R}$, based on the distribution of existing tree samples.
%     \item Construct a set of samples $V_F$ for propagation, selecting samples according to the probability \textbf{$\text{Accept}(\mathcal{R}_i)$} associated with their corresponding region.
%     \item Propagate $V_F$, using \textbf{$\text{Accept}(\mathcal{R}_i)$} to guide the addition of newly generated samples to $\mathcal{T}$.
%     \item Update \textbf{$\text{FreeVol}(\mathcal{R}_i)$} and \textbf{$\text{Cov}(\mathcal{R}_i)$} based on the information gathered during exploration by the sampling-based motion planner.
% \end{itemize}

% The algorithm proceeds by expanding the tree outward through the state space, prioritizing unvisited regions. However, all samples are still considered for expansion. The algorithm manages the samples in three sets: $V_{unexplored}$, $V_{open}$, and $V_F$. $V_{unexplored}$ consists of newly generated samples that have not yet been added to the tree. $V_{open}$ includes samples that are not currently considered for expansion; intuitively these samples lie in regions with low \textbf{$\text{Accept}(\mathcal{R}_i)$} values and are in densely populated areas of the state space. $V_F$ is the current frontier, consisting of tree samples that will be expanded in parallel. The algorithm begins by adding only $x_{init}$ to $V_F$, setting $V_{open}$ and $V_{unexplored}$ to empty and initializing $\mathcal{T}$ with $x_{init}$ at its root. The set $V_F$ is then expanded in parallel where the amount of parallelism is controlled by a parameter $\lambda$, referred to as the branching factor, which dictates how many propagations occur for each sample in $V_F$. The tradeoff for this parameter is as follows: with a low $\lambda$ (i.e., $\lambda \rightarrow 1$), propagation iterations progress quickly, resulting in a sparse tree. However, in early iterations, when $V_F$ is small, this under utilizes the GPU’s parallelism. Conversely, with a high $\lambda$ (i.e., $\lambda \rightarrow 32$), the tree expands rapidly, better utilizing the GPU. But as $V_F$ grows large, the required propagation may exceed the GPU’s capacity, leading to serialized operations. To properly manage $\lambda$ for the specific user's device and problem dynamics, a tuning value $t_e$, referred to as the expected tree size, is introduced to control $\lambda$ for each iteration of parallel expansion. In early iterations, when the tree size $t$ is much smaller than $t_e$, a larger $\lambda$ is used to better utilize the GPU's parallelism and accelerate tree propagation. As the tree size $t$ approaches $t_e$ and $V_F$ becomes large, a smaller $\lambda$ is employed to prevent serialization of the propagation process. If the tree size exceeds $t_e$, the value of $t_e$ is adjusted, setting $t_e = t + t_e$ to accommodate the growing tree and maintain effective parallel expansion. The performance variation when choosing $t_e$ is studied in Section [BLANK] but is shown to be relatively constant for a specific GPU and dynamic system across different environments.

% With the set of samples $V_F$ in hand, each sample is propagated $\lambda$ times, generating a total of $\lambda \times f$ nodes, where $f$ represents the number of samples in $V_F$. The validity of each propagation trajectory is then checked to ensure it is dynamically feasible and free from obstacles. Although checking the validity of each propagation may introduce thread divergence—some threads may encounter collisions earlier than others, leading to idle threads—the information on invalid trajectories is vital for guiding future expansions. Next, the region $\mathcal{R}_i$ and subregion $\mathcal{R}2_j$ are determined for each newly generated node. The counts of valid and invalid samples in each region of $\mathcal{R}$ are updated accordingly. If the sample is valid and its corresponding subregion $\mathcal{R}2_j$ is either unvisited or with a probability equal to its mapped region's acceptance probability, the sample is added to $V{unexplored}$. After all frontier samples have been expanded, the \textbf{$Cov(\mathcal{R}_i)$}, \textbf{$FreeVol(\mathcal{R}_i)$}, and \textbf{$Accept(\mathcal{R}_i)$} values are updated in parallel for each region in $\mathcal{R}$. Once these updates are complete, each sample $x_i \in V_F$ is removed from $V_F$ with a probability determined by one minus
%  \textbf{$Accept(\text{getRegion}(x_i))$} and placed in $V_{open}$, Nodes in $V_{open}$ are added to $V_F$ based on their region's acceptance probability and samples from $V_{unexplored}$ are then removed and added to $V_F$ and $\mathcal{T}$. The algorithm terminates when either a user-defined time limit $t_{max}$ is surpassed or when a node in $\mathcal{T}$ reaches the goal region $X_{goal}$.

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/VisualExplanation/Iteration1.pdf}
        \caption{}
        \label{fig:iteration1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/VisualExplanation/Iteration2.pdf}
        \caption{}
        \label{fig:iteration2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/VisualExplanation/Iteration3.pdf}
        \caption{}
        \label{fig:iteration3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/VisualExplanation/Iteration4.pdf}
        \caption{}
        \label{fig:iteration4}
    \end{subfigure}
    \caption{Illustration of a single iteration in the \alg expansion process. (a) The current sets $V_F$ (in pink) and $V_{open}$ (in blue) are displayed, with the numbers in each grid cell representing the value of \textbf{$\text{Accept}(\mathcal{R}_i)$}. (b) The expansion of each node in $V_F$ is shown, with $\lambda = 2$. (c) The pruning of invalid or less desirable newly generated nodes is depicted, along with the subsequent update of \textbf{$\text{Accept}(\mathcal{R}_i)$} based on the latest expansion data. (d) The updated set $V_F$ is shown, which will be used for expansion in the next iteration.}
    \label{fig:iteration_grid}
\end{figure*}


% \begin{algorithm}[t]
% \caption{\texttt{KGMT}}
% \Require $x_{init}, X_{goal}, t_{max}$
% \State Place $x_{init}$ in $V_F$ 
% \State Set $V_{unexplored}, V_{open}$ to empty.
% \State Initialize $\mathcal{T}$ with root node $x_{init}$.
% \State For each $\mathcal{R}_i$ in $\mathcal{R}$ initialize  \textbf{$\text{Accept}(\mathcal{R}_i)$} to $1$, 
% $n_{invalid}(\mathcal{R}_i)$, $n_{invalid}(\mathcal{R}_i)$ to $0$.
% \State Initialize each region $\mathcal{R}2_i$ in $\mathcal{R}2$ to unvisited.
% \While{$ElapsedTime < t_{max}$}
% \State $\texttt{PropagateFrontier}(V_F, V_{unexplored}, \mathcal{R}, \mathcal{R}2, \lambda)$
% \State $\texttt{UpdateEstimates}(\mathcal{R})$
% \State $\gamma \gets \texttt{UpdateTreeSearch}(V_{unexplored}, V_F, V_{open}, \mathcal{T}, \mathcal{R} X_{goal})$
% \If{$\gamma \neq \text{null}$}
%     \State \Return $\gamma$
% \State \Return $null$
% \end{algorithm}

\begin{algorithm}[t]
    \caption{\alg}
    \label{algo: alg}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{$x_{init}, X_{goal}, t_{max}$}
    \Output{Solution trajectory $\gamma$}
    
    \SetKwFunction{PropagateFrontier}{PropagateFrontier}
    \SetKwFunction{UpdateEstimates}{UpdateEstimates}
    \SetKwFunction{UpdateTreeSearch}{UpdateTreeSearch}
    
    $V_F \gets \{x_{init}\}$ \\
    $V_{unexplored}, V_{open} \gets \emptyset$ \\
    $\mathcal{T} \gets$ Initialize tree with root node $x_{init}$ \\
    
    For each region $\mathcal{R}_i$ in $\mathcal{R}$, set $\text{Accept}(\mathcal{R}_i) = 1$, $n_{invalid}(\mathcal{R}_i) = 0$, and $n_{valid}(\mathcal{R}_i) = 0$.

    For each region $\mathcal{R}2_i$ in $\mathcal{R}2$, mark $\mathcal{R}2_i$ as unvisited.

    \While{$ElapsedTime < t_{max}$}{
        \PropagateFrontier{$V_F, V_{unexplored}, \mathcal{R}, \mathcal{R}2, \lambda$} \\
        \UpdateEstimates{$\mathcal{R}$} \\
        $\gamma \gets$ \UpdateTreeSearch{$V_{unexplored}, V_F, V_{open}, \mathcal{T}, \mathcal{R}, X_{goal}$} \\
        
        \If{$\gamma \neq null$}{
            \KwRet{$\gamma$}
        }
    }
    
    \KwRet{$null$}
\end{algorithm}

\begin{algorithm}[t]
    \caption{PropagateFrontier}
    \label{algo: PropagateFrontier}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{$V_F, V_{unexplored}, \mathcal{R}, \mathcal{R}2, \lambda$}
    \Output{Updated $V_{unexplored}$}
    \tcc{Parallelized GPU Process}
    \ForEach{$x_0 \in V_F$}{
        \For{$i = 1, \dots, \lambda$}{
            Propagate $x_0$, generating $x_1$ \;
            Map $x_1$ to regions $\mathcal{R}_i$ and $\mathcal{R}2_j$ \;
            
            \If{the trajectory from $x_0$ to $x_1$ is valid}{
                Increment $n_{valid}(\mathcal{R}_i)$ \;
                \If{$\mathcal{R}2_j$ is unvisited \textbf{or} $uniform(0,1) \leq Accept(\mathcal{R}_i)$}{
                    Add $x_1$ to $V_{unexplored}$ \;
                }
            }
            \Else{
                Increment $n_{invalid}(\mathcal{R}_i)$ \;
            }
        }
    }
\end{algorithm}

\begin{algorithm}[t]
    \caption{UpdateEstimates}
    \label{algo:UpdateEstimates}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$\mathcal{R}$}
    \Output{Updated estimates for each region $\mathcal{R}_i$}

    \tcc{Parallelized GPU Process}
    \ForEach{$\mathcal{R}_i \in \mathcal{R}$}{
        \texttt{UpdateFreeVol}($\mathcal{R}_i$)\;
        \texttt{UpdateCoverage}($\mathcal{R}_i$)\;
    }

    \tcc{Parallelized GPU Process}
    \ForEach{$\mathcal{R}_i \in \mathcal{R}$}{
        \texttt{UpdateAccept}($\mathcal{R}_i$)\;
    }
\end{algorithm}

\begin{algorithm}[t]
    \caption{UpdateTreeSearch}
    \label{algo:UpdateTreeSearch}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$V_{unexplored}, V_F, V_{open}, \mathcal{T}, \mathcal{R}, X_{goal}$}
    \Output{Trajectory if a goal is found, otherwise $null$}

    \tcc{Parallelized GPU Process}
    \ForEach{$x \in V_F$}{
        Map $x$ to $\mathcal{R}_i$\;
        \If{$uniform(0,1) < 1 - Accept(\mathcal{R}_i)$}{
            Remove $x$ from $V_F$ and place in $V_{open}$\;
        }
    }

    \tcc{Parallelized GPU Process}
    \ForEach{$x_1 \in V_{unexplored}$}{
        Remove $x_1$ from $V_{unexplored}$ and place in $V_F$, $\mathcal{T}$\;
        \If{$x_1 \in X_{goal}$}{
            \Return Trajectory from $\mathcal{T}$ root to $x_1$\;
        }
    }

    \tcc{Parallelized GPU Process}
    \ForEach{$x \in V_{open}$}{
        Map $x$ to $\mathcal{R}_i$\;
        \If{$uniform(0,1) \leq Accept(\mathcal{R}_i)$}{
            Remove $x$ from $V_{open}$ and place in $V_F$\;
        }
    }

    \Return $null$
\end{algorithm}
